Building Implicit Vector Representations of Individual Coding Style

With the goal of facilitating team collaboration, we propose a new approach to building vector representations of individual developers by capturing their individual contribution style, or coding style. Such representations can find use in the next generation of software development team collaboration tools, for example by enabling the tools to track knowledge transfer in teams. The key idea of our approach is to avoid using explicitly defined metrics of coding style and instead build the representations through training a model for authorship recognition and extracting the representations of individual developers from the trained model. By empirically evaluating the output of our approach, we find that implicitly built individual representations reflect some properties of team structure: developers who report learning from each other are represented closer to each other.

==> sections/background.tex <==
\section{Background and motivation}
*mention \cite{azcona2019user2code2vec}*
*mention the LSTM-authorship*

Many of the existing methods of repository analysis, including methods based on machine learning, are crafted for potential use in software engineering tools. *applications; they are mostly related to the technical part*

*mention socio-technical congruence~\citep{cataldo2008socio}: social aspects in teams are manifested in technical artifacts, and this can be assessed with  techniques~\citep{valetto2007using}

Some research had been dedicated to analysis of dynamic interpersonal processes in teams.~\citep{} Moreover, developers report that their use of team collaboration tools, such as code review tools, is not only related to technical artifacts (by resulting in improved code quality), but is also a vital part of interpersonal communication in teams.~\citep{bacchelli2013expectations}

However, modern software engineering tools *do not support social processes*

==> sections/reproducibility.tex <==
\section{Reproducibility}
We make available the technical artifacts of this work: the pipeline to build the representations and data analysis code that we used to map the survey results to the data.
\todo{clean up and upload package to Zenodo}
